Computational analysis of single rising bubbles influenced by soluble surfactant

This paper presents novel insights about the influence of soluble surfactants on bubble flows obtained by Direct Numerical Simulation (DNS). Surfactants are amphiphilic compounds which accumulate at fluid interfaces and significantly modify the respective interfacial properties, influencing also the overall dynamics of the flow. With the aid of DNS local quantities like the surfactant distribution on the bubble surface can be accessed for a better understanding of the physical phenomena occurring close to the interface. The core part of the physical model consists in the description of the surfactant transport in the bulk and on the deformable interface. The solution procedure is based on an Arbitrary Lagrangian-Eulerian (ALE) Interface-Tracking method. The existing methodology was enhanced to describe a wider range of physical phenomena. A subgrid-scale (SGS) model is employed in the cases where a fully resolved DNS for the species transport is not feasible due to high mesh resolution requirements and, therefore, high computational costs. After an exhaustive validation of the latest numerical developments, the DNS of single rising bubbles in contaminated solutions is compared to experimental results. The full velocity transients of the rising bubbles, especially the contaminated ones, are correctly reproduced by the DNS. The simulation results are then studied to gain a better understanding of the local bubble dynamics under the effect of soluble surfactant. One of the main insights is that the quasi-steady state of the rise velocity is reached without ad- and desorption being necessarily in local equilibrium.

==> sections/4_validation.tex <==
%--------------
% Section: Validation and Verification
%--------------
%
\section{Validation}
\label{sec:validation}
The validation of the pure hydrodynamics has been conducted comparing with the experimental data by Duineveld~\cite{duineveld1995} for single bubbles rising in pure water and can be found in~\cite{pesciSPP2017}. \textcolor{blue}{The validation for the sorption source term for fast and slow sorption processes can be found~\cite{pesciSPP2017}, too. The validation of the SGS model with respect to the 2D model problem and for spherical bubbles at small Reynolds numbers (axisymmetric species transfer with a given velocity field) can be found in appendix~\ref{subsec:app_3_a}. In this section we focus on the validation of the implicit SGS model formulation within the interface tracking framework.}


%--------------
\subsection{Subgrid-Scale model for species transfer}
\label{subsec:val_2}
\textcolor{blue}{To validate the solution of the species transfer problem with SGS modelling, the case of a spherical bubble at small Reynolds number is considered. The local Sherwood number $\operatorname{Sh_{loc}}$ is considered for comparison with the reference solution. The local Sherwood number is computed as 
\begin{equation}
\operatorname{Sh_{loc}}(y_i) = \left( \partial_n c \right)_{f_i^{\Sigma}}\ \frac{L_{\mathrm{ref}}}{c_{|\Sigma,c_i} - c_{\infty}}
\label{eq:v15}
\end{equation}
% 
with the normal gradient $\left( \partial_n c \right)_{f_i^{\Sigma}}$ at the interface\footnote{Without the SGS model the gradient is computed as $\left( \partial_n c \right)_{f_i^{\Sigma}} = \left(c_{|\Sigma,c_i} - c_{f_i^{\Sigma}}\right)/d_i$, where $d_i$ is the distance between the boundary face center and the boundary cell center, and $c_{f_i^{\Sigma}}$ is the concentration at the interface face; otherwise $\left( \partial_n c \right)^{SGS}_{f_i^{\Sigma}}$ is used.},the reference length $L_{\mathrm{ref}}$, the concentration in the boundary cell center $c_{|\Sigma,c_i}$ and the species concentration far away from the interface $c_{\infty}$.}

\textcolor{blue}{As a reference, the semi-analytical solution presented in appendix~\ref{subsubsec:app_val_2_2} is used. See appendix~\ref{subsubsec:app_val_2_2} also for the full set of validation results.}

Two different molecular diffusivities are considered corresponding to Schmidt numbers of $\operatorname{Sc} = 10^4,\ 10^7$, where $\operatorname{Sc}$ is the ratio between viscous and molecular diffusion $\nu/D$. The bubble radius is $r_{\mathrm{b}} = 1$ mm and the Reynolds number is set to $\operatorname{Re} = 0.56$. \textcolor{blue}{The local Sherwood number $\operatorname{Sh_{loc}}(\theta_i)$ is computed according to equation~\eqref{eq:v15},} where $\theta_i$ is the polar angle, i.e.~the angle following a streamline on the bubble surface from the top $(\theta = 0)$ to the bottom $(\theta = \pi)$. The bubble equivalent diameter $d_{eq}$ is taken as reference length.

The full 3D problem, hydrodynamics and species transfer from a rising bubble, is solved within the Interface-Tracking framework, see the algorithm in figure~\ref{fig:n5}. 
The computational domain is divided into two sub-domains, one representing the gas phase and the other one representing the liquid phase. The two sub-domains are coupled at the interface via the transmission conditions~\eqref{eq:m3}--\eqref{eq:m5}. The meshes used for the simulations consist of polyhedral cells in the gas phase and prismatic cells with polyhedral base in the bulk phase, as can be seen in figure~\ref{fig:v8}. The interface consists of polyhedral faces with edge length around 50 $\mu m$ and a first cell layer thickness of $l = 12\ \mu$m and $l = 25\ \mu$m. The initial shape of the bubble is a sphere of radius $r_b = 1\ \mathrm{mm}$, the bubble is positioned in the center of a spherical domain of radius $10 r_b$. The calculation is performed in a moving reference frame (MRF) that follows the bubble center during its rise, while the interface is deformable. This last feature is not relevant for the Satapathy-Smith case, because due to the choice of the fluid properties, the bubble does not deform significantly. The presence of a non-inertial reference frame located in the center of the bubble is taken into account via the correction of the momentum equation ($\rho \mathrm{\vec{a}_{MRF}}$ added to the momentum equation) and the velocity boundary condition at the outer domain boundary, $\vec{v}_{\mathrm{out}} = - \vec{v}_{\mathrm{MRF}}$.

\textcolor{blue}{The species concentration at the interface $\Sigma$ is set to $c|_{\Sigma} = 1\ \mathrm{mol/m^3}$, while the initial bulk concentration in $\Omega$ is set to $c_0 = c_{\infty} = 0$.}
The fluids' properties are given in table~\ref{tab:tv1}. Note that the calculated velocity profile in the interface-tracking framework slightly differs from the Satapathy-Smith solution (less than 1.2\%, see~\cite{weberPhD2016}~(section 4.1.2 in the reference)) because the latter refers to a Stokes flow. This small difference can have some impact on the concentration profile close to the interface.
%
\begin{table}[ht]
\caption{Fluid properties for the Satapathy-Smith case.}
\label{tab:tv1}
\centering
\begin{tabular}{ccccccc}
\toprule
$\rho^+\ \mathrm{kg/m^3}$ & $\rho^-\ \mathrm{kg/m^3}$ & $\mu^+\ \mathrm{kg/(ms)}$ & $\mu^-\ \mathrm{kg/(ms)}$ & $\sigma_0\ \mathrm{N/m}$\\
% $\mathrm{kg/m^3}$ & $\mathrm{kg/m^3}$ & $\mathrm{kg/(ms)}$ & $\mathrm{kg/(ms)}$ & $\mathrm{N/m}$\\
\midrule
$1000$ & $1.1965$ & $0.1$ & $1.8 \cdot 10^{-5}$ & $0.0724$\\
\bottomrule
\end{tabular}
\end{table}
\FloatBarrier
%
In figure~\ref{fig:3Dsh} the results in terms of Sherwood number for the 3D case are reported. As can be seen from the two graphs there is a good agreement between the reference solution and the numerical one employing the SGS model. As anticipated, the reference solution is computed based on the Satapathy-Smith velocity profile, thus, since we are dealing with highly non-linear functions (species concentration close to $\Sigma$), small deviations in the velocity field could be enough to produce the observed discrepancies in the results. \textcolor{blue}{In figure~\ref{fig:3Dsh} also the results without the SGS model are plotted.
For small Schmidt numbers, figure~\ref{fig:sc4a3D}, the standard discretization provides results (gray symbols) in good agreement with the reference solution, while the Sherwood numbers resulting from the SGS modelling show a sensitivity to the mesh resolution. On the other hand, for high Schmidt numbers and the given mesh resolution, figure~\ref{fig:sc7a3D}, the standard discretization provides underestimated Sherwood numbers, while the ones obtained with the SGS model are in good agreement with the reference.}
%
\begin{figure}[ht]
\centering
\subfloat[][\emph{Full domain}.]
{\includegraphics[width=.45\textwidth]{./figures/validation/v8_a.png}\label{fig:v8a}} \quad
\subfloat[][\emph{Enlarged view of the bubble region}.]
{\includegraphics[width=.45\textwidth]{./figures/validation/v8_b.png}\label{fig:v8b}}
\caption{3D computational domain for a rising bubble. Inner, outer and surface (dark grey on the right) meshes.}
\label{fig:v8}
\end{figure}
\FloatBarrier
%
%
\begin{figure}[ht]
\centering
\subfloat[][\emph{Sc = 10$^4$}.]
{\includegraphics[angle=-90,width=.488\textwidth]{./figures/validation/Sc4_3D_LINvsSGS}\label{fig:sc4a3D}} \quad
\subfloat[][\emph{Sc = 10$^7$}.]
{\includegraphics[angle=-90,width=.488\textwidth]{./figures/validation/Sc7_3D_LINvsSGS}\label{fig:sc7a3D}}
\caption{Local Sherwood numbers for the species transfer problem with Satapathy-Smith set-up. Black symbols: with SGS modeling, grey symbols: linear interpolation.}
\label{fig:3Dsh}
\end{figure}
\FloatBarrier
%




%--------------
